A Federated Channel Modeling System using Generative Neural Networks

The paper proposes a data-driven approach to air-to-ground channel estimation in a millimeter-wave wireless network on an unmanned aerial vehicle. Unlike traditional centralized learning methods that are specific to certain geographical areas and inappropriate for others, we propose a generalized model that uses Federated Learning (FL) for channel estimation and can predict the air-to-ground path loss between a low-altitude platform and a terrestrial terminal. To this end, our proposed FL-based Generative Adversarial Network (FL-GAN) is designed to function as a generative data model that can learn different types of data distributions and generate realistic patterns from the same distributions without requiring prior data analysis before the training phase. To evaluate the effectiveness of the proposed model, we evaluate its performance using Kullback-Leibler divergence (KL), and Wasserstein distance between the synthetic data distribution generated by the model and the actual data distribution. We also compare the proposed technique with other generative models, such as FL-Variational Autoencoder (FL-VAE) and stand-alone VAE and GAN models. The results of the study show that the synthetic data generated by FL-GAN has the highest similarity in distribution with the real data. This shows the effectiveness of the proposed approach in generating data-driven channel models that can be used in different regions

==> config.tex <==
\usepackage[english]{babel}
%\usepackage[singlelinecheck=false, font=small]{caption}


%\IfFileExists{/etc/motd}{}{\usepackage{epstopdf}}

%\def\baselinestretch{1.}
%\def\baselinestretch{0.93}

\newcommand{\ie}{\emph{i.e.}}
\newcommand{\eg}{\emph{i.e.}}
\newcommand{\etc}{\emph{etc.}}
\newcommand{\ltl}{\gls{ltl}}
\newcommand{\always}{\square}
\newcommand{\eventually}{\Diamond}

\providecommand{\next}{\bigcirc}
\renewcommand{\next}{\bigcirc}

\renewcommand{\land}{\wedge}
\newcommand{\until}{\mathcal{U}}

\newcommand{\todo}[1]{{\textcolor{red}{#1}}}
\newcommand{\clarify}[1]{{\textcolor{orange}{#1}}}


\newenvironment{squishlist}
{\begin{list}{$\bullet$}
    {%
			\setlength{\itemsep}{0pt}%
			\setlength{\parsep}{3pt}%
			\setlength{\topsep}{2pt}%
			\setlength{\partopsep}{0pt}%
			\setlength{\leftmargin}{1.5em}%
			\setlength{\labelwidth}{1em}%
			\setlength{\labelsep}{0.5em}%
	}%
}
{%
	\end{list}%
}

\newenvironment{squishenum}
{
    \begin{list}{$\bullet$}
    {%
			\setlength{\itemsep}{0pt}%
			\setlength{\parsep}{3pt}%
			\setlength{\topsep}{2pt}%
			\setlength{\partopsep}{0pt}%
			\setlength{\leftmargin}{1.5em}%
			\setlength{\labelwidth}{1em}%
			\setlength{\labelsep}{0.5em}%
	}%
}%
{%
	\end{list}%
}

\usepackage{amssymb}
